Delving into the Continuous Domain Adaptation

Existing domain adaptation methods assume that domain discrepancies are caused by a few discrete attributes and variations, e.g., art, real, painting, quickdraw, etc. We argue that this is not realistic as it is implausible to define the real-world datasets using a few discrete attributes. Therefore, we propose to investigate a new problem namely the Continuous Domain Adaptation (CDA) through the lens where infinite domains are formed by continuously varying attributes. Leveraging knowledge of two labeled source domains and several observed unlabeled target domains data, the objective of CDA is to learn a generalized model for whole data distribution with the continuous attribute. Besides the contributions of formulating a new problem, we also propose a novel approach as a strong CDA baseline. To be specific, firstly we propose a novel alternating training strategy to reduce discrepancies among multiple domains meanwhile generalize to unseen target domains. Secondly, we propose a continuity constraint when estimating the cross-domain divergence measurement. Finally, to decouple the discrepancy from the mini-batch size, we design a domain-specific queue to maintain the global view of the source domain that further boosts the adaptation performances. Our method is proven to achieve the state-of-the-art in CDA problem using extensive experiments. The code is available at https://github.com/SPIresearch/CDA.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> suppFolder/abla.tex <==
\begin{table*}[t]
\small
% \vspace{-3mm}
\centering
\caption{Analysis Results (\%) in Small Norb Dataset.}
% \fontsize{7.7}{8.5}\selectfont
% \setlength\tabcolsep{0.55pt}
\begin{tabular}{lrrrrrrrrrrrrrr}
\hline 
\multirow{2}{*}{Method}&  P 1& \multicolumn{4}{c}{P 2} & \multicolumn{4}{c}{P 3} & \multicolumn{4}{c}{P 4}& \multirow{2}{*}{Avg.}\\
   & S 1&S 1   &S 2     &S 3     &S 4    &S 1     &S 2     &S 3     &S 4    &S 1     &S 2     &S 3     &S 4  \\
\hline  
 Variant 1 &  88.6&  87.2&     87.1&     87.4&    88.8&  88.2&    87.3&     86.4&    86.4&   87.7&    86.5& 86.4& 87.3& 87.3 \\
 Variant 2 &  83.4&    87.6&     87.5&     86.4&    87.1&  84.0&    84.2&     85.5&    86.8&   83.5&    85.6&     85.6& 87.1&85.7\\
 Variant 3 &  88.1&    86.6&     88.4&     88.0&    87.3&  88.3&    87.4&     85.7&    87.5&   86.5&    88.2&     86.6& 87.6 &87.4\\
 Variant 4 &  86.4&    86.7&     88.5&     86.0&    87.2&  85.2&    86.6&     85.8&    87.8&   85.1&    86.7&     85.6& 87.0 &86.5\\
 Variant 5 &  83.4&    85.1&     85.4&     82.5&   87.0 &  85.9&    87.5&     84.5&    86.4&   86.5&    87.3&     84.5& 86.5&85.6\\
 Variant 6 &  90.2&    86.5&     89.7&     88.9&   89.0 &  87.5&    89.3&     87.4&    89.1&   88.7&    89.1&     87.5 & 89.3&88.6\\
 Variant 7 &  89.8&    89.1&     89.1&    88.3&  88.0 &  89.1&    89.1&     88.8&    88.1&   87.9&    87.9&     85.9&  87.6& 88.4\\
\hline  
Ours & \textbf{91.5}&    \textbf{90.5}&  \textbf{90.3}&     \textbf{89.6}&    \textbf{89.8}&  \textbf{87.6}&    \textbf{89.5}&     \textbf{87.4}&    \textbf{89.7}&   \textbf{87.8}&    \textbf{89.4}&     \textbf{87.8}& \textbf{90.1}& \textbf{89.3}\\
\hline
\end{tabular}

\label{analy}
\end{table*}

==> suppFolder/analysis.tex <==
\section{Analysis and Discussion}

\subsection{Motivation Clarifications}

We clarify and re-emphasize essential motivations of the new CDA task and the proposed method. 

\textbf{Motivation of the CDA Formulation.} The novel CDA problem is analogous to practical setting where we are given a dataset in the real-world application with a continuously varying attribute. Furthermore, such attribute variations, although sometimes tiny, will destroy the model developed using partially annotated data obtained from the dataset. In the CDA task, all domains are sampled based on the continuous attribute and the domain variations are mainly caused by the attribute variations. The task is practical as we are only given two source domains with data and annotations and the un-annotated probe target domain data, with the goal of learning a generalized model using these information. Note that the test data also comprises unseen domains. 

\textbf{Motivation of the Alternating Direction Training Strategy.} The main objective of CDA is to learn a generalized model tackling discrepancies among all domains sampled on a continuous attribute. To handle the statistics of unseen domain data, our strategy is to study the geometry of the continuous attribute and use it as an inductive bias in the modelling. Inspired by this principle, we design the alternating direction training strategy, including two steps: Pull and Shrinkage. In P step, we regard the trajectory formed by the two source domains as the inductive bias and pull target domains to the trajectory so that unseen target domains have higher chance to be close to the trajectory as well. In S step, we progressively shrink and shorten the trajectory. Alternating the two steps in the training, the proposed method is proved to be able to generalize to unseen target domains. 

% \begin{figure}[!t]
% \centering
% \includegraphics[width=\columnwidth]{figure/early.pdf}
% \caption{(a)Source-target discrepancy.(b)Source-source discrepancy. Red circles denote the biased discrepancies during early training.}
% \label{ana}
% \end{figure}

\textbf{The definitions of the auxiliary classifier $F'$ and the discrepancy measure.} $F'$ and $F$ are both classifiers with the same architecture and take the same input and outputs. Note that content classifiers $F$ and $F_2$ are used to classify content labels in each source domain, while auxiliary classifiers $F_1'$ and $F_2'$ are used to estimate the discrepancies (together with content classifiers). $p'(\hat{y}|e)$ indicates the probabilities of that $F'$ and $F$ predicting the same class. The discrepancy between $P$,$Q$ is formally defined as: 
\begin{align}
\mathcal{D}(e_P,e_Q) = \sup_{F'}\mathbb{E}_P\log p'(\hat{y}|e) + \mathbb{E}_Q \log(1-p'(\hat{y}|e)).
\end{align}
% \begin{align}
% \mathcal{D}(e_P,e_Q) = \sup_{F'}\mathbb{E}_P\log p'(\hat(y)|e) + \mathbb{E}_Q \log(1-p'(\hat(y)|e)).
% \end{align}
It can be derived into the form of JS divergence(see section 3.3).



%  It can be observed that some methods localize different class-specific image regions in domains. For example, in CIDA, model pays more attention on eyes in two source domains, while in localize forehead in some unseen target domains which leads to misclassification. As for our method(the last row), model shows the same localization, eye, in all domains, and achieve right classifications. The results show that our method can localize the discriminative image regions without the impact of domain shift.  
\subsection{Analysis of the Method Effectiveness}
\textbf{T-SNE Results} In Figure \ref{mis-tsne}, we visualize the T-SNE feature of target, source domains among different training epochs. It can be observed that the source domain features (blue and orange) points are gradually spreading to the grey zone (all target domains). Finally when it comes to epoch 150, and 200, the T-SNE converges. 

\textbf{Detailed Sub-Domain Accuracy} As shown in Table \ref{ana_err}, the sub-domain accuracy is reported in the continuous DA task. It can be observed that our method can not only outperform other methods in unseen target domains (U), probe target domains (P) but also can outperform the source-only model on source domains (S1,S2). It is a very essential observations as it proves that our training strategy works as a specially designed augmentation procedure and helps generalization. 

As it outperforms the supervised learning method on the source domains, it proves that our method won't "forget" the knowledge from the source domain and regard the overall performances in all the continuous domains as the training objective. 

\textbf{Failure Cases} In addition, we present some hard samples and failure cases that are misclassified by all methods in Figure \ref{mis-hard}. We hypothesize that this is mainly due to the poor quality of GAN in the synthesis procedure. The genuine cases of this observation is worth investigations in the future. 


\input{tables/acc_ana}



% \subsection{Insights}


% In addition, we present some hard samples that are misclassified by all methods in Figure \ref{mis}.
% \input{tables/acc_ana}

% - when budgets are limited, how to select the best domains to annotate. 

\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{figure/hard_sample.pdf} 
\caption{Examples that are misclassified by all methods.}.
\label{mis-hard}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{figure/5_tsne.pdf} 
\caption{Visualization of t-SNE in different epochs.}.
\label{mis-tsne}
\end{figure}

\subsection{Theoretical Justifications}
\textbf{Optimization in P step} We first consider the optimization problem we have defined in stage P:
\begin{align}
 \mathcal{D}_{1}(e_{s_1},e_{t_i}) + \mathcal{D}_{2}(e_{s_2},e_{t_i}) \label{dss}\\
 =\sum_{j=1,2}\max_{F_j'}\big[-\mathbb{E}_{e_{s_1}\sim P_{s_j}}\log[\sigma_{h_{F_j}(e)}\circ F'_j(e)]  \notag  \\
 - \mathbb{E}_{e_{t_i}\sim P_{t_i}}\log[1-\sigma_{h_{F_j}(e)} \circ F'_j(e)]\big] \label{eq3}  \notag \\
\end{align}
Let $J_j(e) = \sigma_{h_{F_j}(e)}\circ F'_j(e)$, then,
\begin{align}
&\mathcal{D}_{1}(e_{s_1},e_{t_i}) + \mathcal{D}_{2}(e_{s_2},e_{t_i})  \notag \\
 = &\max_{F_1'} \int_{e}-P_{s_1} \log J_1(e) - {P_{t_i}}\log(1- J_1(e)) de \notag \\
  +&\max_{F_2'} \int_{x} - P_{s_2} \log J_2(e)  - {P_{t_i}}\log(1-J_2(e) ) de
\end{align}
Eq.(3) reaches the largest when
\begin{align}
\label{op1}
 J_1(e) = \sigma_{h_{F_1}(e)}\circ F'_1(e) = \frac{ P_{s_1}}{P_{s_1} + P_{t_i}}\\
 \label{op2}
 J_2(e) = \sigma_{h_{F_2}(e)}\circ F'_2(e) = \frac{ P_{s_2}}{P_{s_2} + P_{t_i}}.
\end{align}
Replace Eq.\eqref{op1} and Eq.\eqref{op2} into Eq.\eqref{dss},
% If we substitute Eq \eqref{op1} into Eq \eqref{alpha1}, the target-source discrepancy is equivalent to a JS-divergence:
% \begin{align}
% \label{js1}
% D_{s,t}(T,S) = \text{JS}(P_{s1}||P_t) + \text{JS}(P_{s2}||P_t) - 4\log{2}
% \end{align}
\begin{align}
&\mathcal{D}_{1}(e_{s_1},e_{t_i}) + \mathcal{D}_{2}(e_{s_2},e_{t_i})  \notag \\
=& \max_{F_1'} \int_{e}-P_{s_1} \log \frac{ P_{s_1}}{P_{s_1} + P_{t_i}} - {P_{t_i}}\log\frac{ P_{t_i}}{P_{s_1} + P_{t_i}} de \notag \\
  + &\max_{F_2'} \int_{x} - P_{s2} \log \frac{ P_{s_2}}{P_{s_2} + P_{t_i}}  - {P_{t_i}}\log\frac{ P_{t_i}}{P_{s_s} + P_{t_i}} de\notag \\
=& JS(P_{s_1}||P_{t_i}) + JS(P_{s_2}||P_{t_i}) + 2\log2
\end{align}
Thus,
\begin{align}
&\min_{E} \mathcal{D}_{1}(e_{s_1},e_{t_i}) + \mathcal{D}_{2}(e_{s_2},e_{t_i})  \notag \\
=& \min_{E} JS(P_{s_1}||P_{t_i}) + JS(P_{s_2}||P_{t_i}) + 2\log2 \notag \\
=& \min_{E} JS(P_{s_1}||P_{t_i}) + JS(P_{s_2}||P_{t_i})
\end{align}
\textbf{Optimization in S step} The optimization problem is defined as follow:
\begin{align}
&\mathcal{D}_{1}(e_{s_1},e_{s_2}) + \mathcal{D}_{2}(e_{s_2},e_{s_1})  \label{dsst} \\
 = &\max_{F_1'} \int_{e}-P_{s_1} \log J_1(e) - {P_{s_1}}\log(1- J_1(e)) de \notag \\
  +&\max_{F_2'} \int_{x} - P_{s_2} \log J_2(e)  - {P_{s_1}}\log(1-J_2(e) ) de
\end{align}
Eq.(9) reaches the largest when
\begin{align}
\label{op11}
 J_1(e) = \sigma_{h_{F_1}(e)}\circ F'_1(e) = \frac{ P_{s_1}}{P_{s_1} + P_{s_2}}\\
 \label{op22}
 J_2(e) = \sigma_{h_{F_2}(e)}\circ F'_2(e) = \frac{ P_{s_2}}{P_{s_1} + P_{t_2}}.
\end{align}
Replace Eq.\eqref{op11} and Eq.\eqref{op22} into Eq.\eqref{dsst},
\begin{align}
&\mathcal{D}_{1}(e_{s_1},e_{s_2}) + \mathcal{D}_{2}(e_{s_2},e_{s_1})\\
=&2JS(P_{s_1}||P_{S_2}) + 4\log2
\end{align}
Thus,
\begin{align}
&\min_{E} \mathcal{D}_{1}(e_{s_1},e_{s_2}) + \mathcal{D}_{2}(e_{s_2},e_{s_1})  \notag \\
=& \min_{E} 2JS(P_{s_1}||P_{s_2}) + 4\log2 \notag \\
=& \min_{E} JS(P_{s_1}||P_{s_2}) \end{align}

\textbf{Global optimum.} Eq.(8) has the minimum at $P_{s_1}=P_{t_i}$ or $P_{s_2}=P_{t_1}$, while Eq.(15) at $P_{s_1}=P_{s_2}$. Thus, two stages has the global optimum at $P_{t}=P_{s_1}=P_{s_1}$.






% stage 1
% \begin{align}
% \max_{f_1',f_2'} d_{f_1,F} (P_{s1},P_t) + d_{f_2,F}(P_{s2},P_t)
% \end{align}

% \begin{align}
%   d_{f_1,F} (P_{s1},P_t) + d_{f_2,F}(P_{s2},P_t) \notag \\
% = \int_{x} P_{s1}\log (\sigma_{h_{f_1}}\circ f_{1}') + P_{t}\log (1-\sigma_{h_{f_1}}\circ f_{2}')\notag \\
% +P_{s2}\log (\sigma_{h_{f_2}}\circ f_{2}') + P_{t}\log (1-\sigma_{h_{f_2}}\circ f_{2}') dx
% \end{align}

% \begin{align}
% \sigma_{h_{f_1}}\circ f_{1}'^{*} = \frac{ P_{s1}}{P_{s1} + P_t}\\
% \sigma_{h_{f_2}}\circ f_{2}'^{*}= \frac{ P_{s2}}{P_{s2} + P_t}
% \end{align}

% \begin{align}
% \min_{f_1,f_2, \phi} d_{f_1,F} (P_{s1},P_t) + d_{f_2,F}(P_{s2},P_t)
% \end{align}

% \begin{align}
%  d_{f_1,F} (P_{s1},P_t) + d_{f_2,F}(P_{s2},P_t)\notag \\
%  = \int_x P_{s1} \log \frac{P_{s1}}{P_{s1}+P_{t}} + P_{t} \log \frac{P_{t}}{P_{s1}+P_{t}} \notag \\
% +P_{s2} \log \frac{P_{s2}}{P_{s2}+P_{t}} + P_{t} \log \frac{P_{t}}{P_{s2}+P_{t}} dx \notag \\
% = \int_x  P_{s1} \log \frac{2P_{s1}}{P_{s1}+P_{t}} + P_{t} \log \frac{2P_{t}}{P_{s1}+P_{t}} \notag \\
% +P_{s2} \log \frac{2P_{s2}}{P_{s2}+P_{t}} + P_{t} \log \frac{2P_{t}}{P_{s2}+P_{t}}  \notag \\
%  - (P_{s1} + P_{s2} +2P_{t}\log{2}) dx  \notag \\
% = JS(P_{s1}||P_t) + JS(P_{s2}||P_t) - 4\log{2}
% \end{align}

% stage 2
% \begin{align}
% \max_{f_1',f_2'} d_{f_1,F} (P_{s1},P_{s2}) + d_{f_2,F}(P_{s1},P_{s2})
% \end{align}

% \begin{align}
%   d_{f_1,F} (P_{s1},P_{s2}) + d_{f_2,F}(P_{s1},P_{s2}) \notag \\
% = \int_{x} P_{s1}\log (\sigma_{h_{f_1}}\circ f_{1}') + P_{s2}\log (1-\sigma_{h_{f_1}}\circ f_{1}')\notag \\
% +P_{s2}\log (\sigma_{h_{f_2}}\circ f_{2}') + P_{s1}\log (1-\sigma_{h_{f_2}}\circ f_{2}') dx
% \end{align}

% \begin{align}
% \sigma_{h_{f_1}}\circ f_{1}'^{*} = \frac{ P_{s1}}{P_{s1} + P_{s2}}\\
% \sigma_{h_{f_2}}\circ f_{2}'^{*}= \frac{ P_{s2}}{P_{s1} + P_{s2}} 
% \end{align}

% \begin{align}
%  &d_{f_1,F} (P_{s1},P_{s2}) + d_{f_2,F}(P_{s1},P_{s2})\notag \\
%  &= \int_x 2P_{s1} \log \frac{P_{s1}}{P_{s1}+P_{t}} + 2P_{s2} \log \frac{P_{s2}}{P_{s1}+P_{s2}}  dx \notag \\
% &= \int_x  2P_{s1} \log \frac{2P_{s1}}{P_{s1}+P_{t}} + 2P_{s2} \log \frac{2P_{t}}{P_{s1}+P_{t}} \notag \\
%  &- (2P_{s1} + 2P_{s2})\log(2) dx  \notag \\
% &= 2JS(P_{s1}||P_{s2}) - 4\log{2}
% \end{align}

% \begin{align}
% \label{12}
% d_{f_1,F} (P_{s1},P_t) + d_{f_2,F}(P_{s2},P_t) \notag \\ -\frac{1}{2}(d_{f_1,F} (P_{s1},P_{s2}) + d_{f_2,F}(P_{s1},P_{s2})) + 2\log{2}\notag \\
% = JS(P_{s1}||P_t) + JS(P_{s2}||P_t) - JS(P_{s1}||P_{s2})
% \end{align}
% when $JS(P_{s1}||P_{s2})$ small enough, \ref{12} $\leq0$, equality holds when $P_s1=P_s2=P_s3$

==> suppFolder/complex.tex <==
\begin{table*}[!t]
\centering
\small

\setlength\tabcolsep{0.55pt}
%\resizebox{0.85\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c}
\toprule
 Method &Backbone& Params(M) &FLOPs(M) &Backbone& Params(M) &FLOPs(M)\\
 \midrule
 DRT& \multirow{2}{*}{4-layer CNN}&1.86& 0.23& \multirow{2}{*}{ResNet-50} &29.5& 6.45\\
Ours & &1.59&0.048& &23.5& 5.38\\
\bottomrule
\end{tabular}
%}
\caption{Complexity analysis.}
\label{complexity}
\end{table*}

==> suppFolder/dataset_analysis.tex <==
\section{Dataset Analysis}
We conduct an in-depth analysis of the cross-domain statistics in three dataset in Figure \ref{data}. Three results are reported including the 1) target domain performances using different source-only models; 2) average target domain performances of source-only models; 3) MMD \cite{tolstikhin2016minimax} between source and target domain features using pre-trained source-only model. 
\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{figure/data_ana.pdf}
\caption{Analysis including target domain accuracy, average target domain accuracy and MMD between source and target domains. }.
\label{data}
\end{figure}
% We successively train the model on each domain as source domain and perform adaptation on the whole test set. We record the accuracy on each domain and the average accuracy. Additionally, we visualize the MMD \cite{NIPS2016_5055cbf4} between source and each target domain. 


% We conduct an in-depth analysis of the cross-domain statistics in CONDA benchmark. We successively train the model on each domain as source domain and perform adaptation on the whole test set. We record the accuracy on each domain and the average accuracy. Additionally, we visualize the MMD \cite{NIPS2016_5055cbf4} between source and each target domain. The results are shown in Figure \ref{anafig}.

From the Figure \ref{data} (a)(d)(g), we made two observations: \textit{first}, the performance of each source domain model(a plot using a specific color) reaches the peak at the source attribute but successively drops when the attribute keeps moving far away from the source one. This suggests that the domain shift increases with the increasing attribute differences. \textit{Second}, smallNORB and Face Age Synthesis exhibit the similar smooth performance patterns among all target domains, however, the performance curve in EMNIST has a very steep peak point on the source attribute and performances drop very quickly for other attributes/domains. This suggests that current deep network architecture is not suitable to tackle rotation variations and the domain gaps in this dataset seem the largest. 
% large performance gaps can be observed between source and target domains, even if the attribute differences are small and domains are close (See Figure \ref{anafig} (b) as an example).
It confirms the fact that deep architectures cannot tackle the domain shift in CDA. 
% By looking at the left figures of Figure \ref{anafig} (a),(b),(c), several observations can be made. First, the accuracy reach peak at the source domain and gradually drops. It is reasonable that the distribution continuously changes with the attribute. As a consequence, the domain shift increase with the difference of attribute. Second, there is a large performance gap between source and target domains. It confirms the fact that deep architectures do not solve the domain shift problem. 
In the Figure \ref{data} (b)(e)(h), smallNORB and Face Age Synthesis exhibit the similar average performances patterns among all target domains, where the performance first rises and then falls. Instead, the performance curve in EMNIST is stable among different attributes. It is reasonable because deep networks are not able to handle rotation variations.
% It can be explained from the information perspective. 
% We categorize the dataset according to the information of domains, as shown in Figure \ref{datainf}. The first category (Figure \ref{datainf} (a)) is smallNORB, each domain contain a part of information of the whole continuous domain, and overlap exists between adjacent domains. Domains in the middle share more information so they achieve better performance. 
% While EMNIST is categorized into Figure \ref{datainf} (b). Although domains are characterized by rotation angles, they contains the same information. Thus, they show similar adaptation performances. 
% The results of Face Age Synthesis is similar with smallNORB, but there is still some differences. As people grow, some characteristics of appearance keep invariable, such as complexion, hair curvature,  pupil color, which cause all domains share a part of information, as shown in Figure \ref{datainf} (c). 

Finally, it is observed in Figure \ref{data} (c)(f)(i) that the closer to the diagonal, the darker the point color is. The phenomenon is strongly correlated to the accuracy curve. It provides the insights that the choice of samples to annotate has an impact on the performance when the annotation budget is limited. 

==> suppFolder/digitda.tex <==
\begin{table}[h]
\centering
\caption{Multi-target DA results (\%) in Digit-Five.}
\small
\begin{tabular}{c|c|c|c|c}
\hline
%'mnist', 'usps',  'syn', 'mnist_m', 'svhn'
%mt, up, sv, sy, mm are abbreviations for MNIST, USPS, SVHN, Synthetic Digits, MNIST-M
Dataset &mt & mm & sv& up \\
& $\rightarrow$up, sy& $\rightarrow$mt,up& $\rightarrow$mt,mm&$\rightarrow$sy,mm\\
\hline
SO & 30.9 &92.0 &51.3 &23.0\\
Ours &34.9 &93.4 &73.0 &41.9\\
\hline
\end{tabular}

\label{mtda}
\end{table}


==> suppFolder/discussion.tex <==
\section{Discussions}

==> suppFolder/result.tex <==
\section{Additional Results}
% To demonstrate our method's universality, we further evaluate on five classic digits datasets \chensays{give a figure here.} (MNIST\cite{lecun1998gradient},USPS\cite{hull1994database}, MNIST-M\cite{ganin2015unsupervised},SynNum\cite{ganin2015unsupervised}, and SVHN\cite{netzer2011reading}). MNIST and USPS are datasets for handwritten digits, while MNIST-M and SynNum are for syntheic numbers. SVHN are collected form street view housing numbers.  All images are resized to $32 \times 32$ and 3 channels. Besides, no further transforms is applied to the data. We designate each dataset as a domain. As there is not a explicit attribute among them, we sort them by the complexity: MNIST, USPS,  SynNum, MNIST-M, SVHN. For each domain, we follow the origin training/testing split. Beacuse of the limited number of domains, we adopt different splits: MNIST and SHVN are used as source domain, and one of the rest three is used as probe target domain. Besides, we record the accuracy of each domain, as the number of samples are unbalance in different domains.



\subsection{More comparison methods}
We compare with other methods, including source-only model with a Maximum Mean Discrepancy (MMD) discrepancy measurement. In addition, we compare with the state-of-the-art Domain Generalization (DG) method, and continual learning method.
\input{suppFolder/supp_norb}

\textbf{Compare with Single-Domain DA modules.}
MMD \cite{tolstikhin2016minimax} is a popular discrepancy measurement in UDA. We adopt to compare with the method using MMD on the source only model to reduce the cross-domain discrepancy. The results are shown in Table \ref{sonorb}, denoted as So+MMD. We can observe that So+MMD leads to degraded performances. We conjecture that MMD failed to measure the discrepancy among source domain and unseen target domains, therefore disturbing the geometry of continuous domains. Consequently, the discrepancy among unseen target domains are enlarged.

\textbf{Compare with DG method.}
Due to similarities to DG methods, we also reproduce the MixStyle \cite{zhou2021mixstyle}, the SOTA DG method which mixes instance-level feature to perform DG. We add the MixStyle module after the third convolution layer of source-only model to mix features from two source domains. The results are shown in Table \ref{sonorb}, denoted as So+MixStyle. It seems that the performances are very close to the So performances. It demonstrates the complexity of the geometry of continuous domain and because of this, the mixture of two source domains cannot approximate the target domains accurately.

\textbf{Compare with Continual learning method.}
We reproduce the continual learning method on the CDA datasets, including Continuous Unsupervised Adaptation(CUA)\cite{bobu2018adapting}, and Evolving domain adaptation(EDA)\cite{NEURIPS2020_fd69dbe2}. The results are shown in Table \ref{sonorb}. It seems that continual learning leads to degraded performances. We conjecture that these methods fail to general on the whole distribution because of ignoring the unseen domains. 


\subsection{More results of ablation study on CDA}
We perform ablation studies on all splits in Small Norb dataset to support the main submission ablation studies. The results are shown in Table \ref{analy}. It verifies the effectiveness of each proposed main contribution, including: 1) the discrepancy measure, 2) the alternating two-stage training strategy, 3) the continuity constraint using gradient plenty, and 4) feature queues. 

\subsection{Evaluation on Existing Multi-Domain Benchmark}
\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{figure/digits.pdf} 
\caption{Examples of C-DIGIT benchmark.}.
\label{dig}
\end{figure}
To demonstrate the effectiveness of our method in other multi-domain adaptation tasks (without continuous attribute variations observed), we evaluate it using the C-DIGIT \cite{compounddomainadaptation} benchmark including five classic digits datasets (as shown in Figure \ref{dig}): MNIST(mt)\cite{lecun1998gradient}, USPS(up)\cite{hull1994database}, MNIST-M(mm)\cite{ganin2015unsupervised}, SynNum(sy)\cite{ganin2015unsupervised}, and SVHN(sv)\cite{netzer2011reading}. Note that although the C-DIGIT dataset is not able to evaluate the continuous DA method, we can use it to evaluate our method handling multiple domain discrepancies caused by discrete and irrelevant domain attribute variations. All images are resized to $32 \times 32$ and 3 channels and no further transforms are applied to the data. We regard each dataset of the five digit ones as a single domain. As the domain attribute and the variations cannot be explicitly observed among these datasets, we sort them by the complexity, assuming that they lie on the continuous attribute space in the following order: MNIST, USPS,  SynNum, MNIST-M, SVHN. Due to the limited domain numbers, we evaluate our method using the following setup: MNIST and SHVN are used as source domain, and one of the rest three is used as probe target domain and the rest target domain is regarded as the unseen test ones. 
% Besides, we report the accuracy of each domain, as the number of samples are unbalance in different domains.

The results are shown in Table \ref{ana_digits}. It seems that the proposed method is able to outperform other comparison methods and can reduce multi-domain discrepancies caused by discrete and irrelevant domain attribute variations. Moreover, we evaluated our method for multi-source and multi-target DA in Table \ref{mtda}. It shows that our method is effective in multi-target DA setting. 

\subsection{Commonality and uniqueness. } From the mentioned comparison and the main submission, we can observe that a few single-domain, multi-source/target DA and DG methods, as well as continual learning method, are applicable to CDA, but achieve worse performances than ours. It shows the \textbf{\textit{uniqueness}} of CDA. In addition, our method is applicable to Multi-Source and Multi-Target DA, achieving SOTA results.  It demonstrates the \textbf{\textit{commonality}} of CDA.

% To demonstrate our method's universality, we further evaluate on five classic digits datasets (as shown in Figure \ref{dig}): \chensays{give a figure here.} MNIST(mt)\cite{lecun1998gradient},USPS(up)\cite{hull1994database}, MNIST-M(mm)\cite{ganin2015unsupervised},SynNum(sy)\cite{ganin2015unsupervised}, and SVHN(sv)\cite{netzer2011reading}. MNIST and USPS are datasets for handwritten digits, while MNIST-M and SynNum are for syntheic numbers. SVHN are collected form street view housing numbers.  All images are resized to $32 \times 32$ and 3 channels. Besides, no further transforms is applied to the data. We designate each dataset as a domain. As there is not a explicit attribute among them, we sort them by the complexity: MNIST, USPS,  SynNum, MNIST-M, SVHN. For each domain, we follow the origin training/testing split. Beacuse of the limited number of domains, we adopt different splits: MNIST and SHVN are used as source domain, and one of the rest three is used as probe target domain. Besides, we record the accuracy of each domain, as the number of samples are unbalance in different domains.
\input{suppFolder/abla}
\input{suppFolder/table_digit}
\input{suppFolder/digitda}




==> suppFolder/supp_norb.tex <==
\begin{table*}[t]
\small
\caption{Comparision Results (\%) in SmallNorb Dataset.}
\centering
% \resizebox{\linewidth}{!}{
\begin{tabular}{c|c|cccc|cccc|cccc|c}
\hline
\multirow{2}{*}{Method}&  P 1& \multicolumn{4}{c|}{P 2} & \multicolumn{4}{c|}{P 3} & \multicolumn{4}{c|}{P 4}& \multirow{2}{*}{Avg.}\\
   & S 1&S 1   &S 2     &S 3     &S 4    &S 1     &S 2     &S 3     &S 4    &S 1     &S 2     &S 3     &S 4  \\
\hline
So &85.1 &88.8 &88.8 &88.8 &88.8 & 86.8 &86.8 &86.8 &86.8 &86.5&86.5&86.5&86.5&87.1\\
So + MMD &78.2 &80.6&82.5 &79.4 &77.4 &80.2 &80.3 &73.8 &72.8 &80.7 &80.1 &78.5&77.0&78.6\\
So + MixStyle &84.0&88.0&88.0&88.0&88.0 &87.1 &87.1 &87.1 &87.1 &87.1 &87.1 &87.1 &87.1&87.1\\
CUA &84.8 & 86.8 &86.4 &83.9 &85.8 &85.5 &87.5 &84.8 &87.4 &82.8 &83.0 &81.0 &85.9 &85.0\\
EDA &45.3 &41.7 &49.0 &65.9 &66.0 &38.1  &42.1 &55.3 &51.8 &39.6 &43.4 &69.9 &65.1 &51.6\\
\hline  
Ours & \textbf{91.5}& \textbf{90.5}& \textbf{ 90.3}&     \textbf{89.6}&    \textbf{89.8}&  \textbf{87.6}&    \textbf{89.5}&     \textbf{87.4}&    \textbf{89.7}&   \textbf{87.8} &    \textbf{89.4}&     \textbf{87.8} &\textbf{90.1} & \textbf{89.3}\\
\hline 
\end{tabular}
% }

\label{sonorb}
\end{table*}


==> suppFolder/table_digit.tex <==
\begin{table}[t]
\centering
\caption{Comparision Results (\%) in five digits datasets.mm and sv are source domains and we test on mm.}
\begin{tabular}{c|c|c}
\hline
\multirow{2}{*}{Method} &\multicolumn{2}{c}{probe target domain}\\
&up & sy \\
\hline
SO &45.4 &45.4\\
CIDA &43.9 &48.6 \\
ATDOC &40.6 &50.1  \\
BCDM &27.6 &40.2\\
\hline 
Ours &\textbf{49.5} &\textbf{53.3}\\
\hline 
\end{tabular}

\label{ana_digits}
\end{table}


% \begin{table*}[t]
% \small
% \caption{Comparision Results (\%) in five digits datasets.\chensays{@yinsong, please change this in priority.}}
% \centering
% \begin{tabular}{c|c|c|c|c}
% \hline 
% Src. Domain& \multicolumn{2}{c|}{up} & \multicolumn{2}{c|}{sy} \\
% \hline 
% mt, sv& mt& up& sy& mm&  sv&  mt& up& sy& mm&  sv&  mt& up& sy& mm&  sv  \\
% \hline  
% SO &99.2&96.7&86.5&45.4&90.3 &99.2&96.1&89.5&45.4&90.3&99.2&96.1&86.5&45.4&90.3\\
% CIDA &93.8&80.6&70.1&43.9&71.5&98.2&92.5&78.9&48.6&84.8 &98.8&93.7&85.9&53.6&88.8\\
% ATDOC &98.3&95.4&73.1&40.6&80.7 &98.9&92.7&83.4&50.1&86.9  &98.1&92.7&75.6&45.2&82.3\\
% BCDM &91.3&25.2&48.5&27.6&68.2 &96.1&88.2&88.3&40.2&82.0&97.4&90.8&89.1&40.7&83.1\\
% DRT &99.1&96.1&83.9&47.7&88.9 &98.7&93.2&79.8&47.19&85.6 &99.1&95.6&84.3&48.9&88.9\\
% \hline  
% Ours &96.2&92.5&72.9&49.5&72.7 &94.3&83.5&76.4&53.3&73.5&89.3&80.6&71.1&55.9&69.6\\
% \hline 
% \end{tabular}
% \label{ana_digits}
% \end{table*}


